Early Prediction for Merged vs Abandoned Code Changes in Modern Code Reviews

The modern code review process is an integral part of the current software development practice. Considerable effort is given here to inspect code changes, find defects, suggest an improvement, and address the suggestions of the reviewers. In a code review process, usually, several iterations take place where an author submits code changes and a reviewer gives feedback until is happy to accept the change. In around 12% cases, the changes are abandoned, eventually wasting all the efforts. In this research, our objective is to design a tool that can predict whether a code change would be merged or abandoned at an early stage to reduce the waste of efforts of all stakeholders (e.g., program author, reviewer, project management, etc.) involved. The real-world demand for such a tool was formally identified by a study by Fan et al. [1]. We have mined 146,612 code changes from the code reviews of three large and popular open-source software and trained and tested a suite of supervised machine learning classifiers, both shallow and deep learning based. We consider a total of 25 features in each code change during the training and testing of the models. The best performing model named PredCR (Predicting Code Review), a LightGBM-based classifier achieves around 85% AUC score on average and relatively improves the state-of-the-art [1] by 14-23%. In our empirical study on the 146,612 code changes from the three software projects, we find that (1) The new features like reviewer dimensions that are introduced in PredCR are the most informative. (2) Compared to the baseline, PredCR is more effective towards reducing bias against new developers. (3) PredCR uses historical data in the code review repository and as such the performance of PredCR improves as a software system evolves with new and more data.

==> implications.tex <==
\section{Implications}
\label{sec:implications}
%implications of findings and the tool.

%\gias{follow this paper (Section 5.6): \url{https://sail.cs.queensu.ca/Downloads/EMSE2019_CharacterizingAndIdentifyingRevertedCommits.pdf}}

%\anindya{Once the results are there, "Usage Scenarios, Benefits, and Costs of our Approach" may be written following the paper above. I have written the other part.}

As described in the Introduction,
the basic usage scenario of our tool is to provide early warnings to authors, reviewers, and the management about
review iterations that will eventually be abandoned. 

\subsection{Implication for Software Project Management}

This tool is likely to provide significant benefits to software project management. If the management can predict the negative outcome of a review-iteration early, they may analyze the cause and take necessary steps if required. Multiple reasons may act behind the abandonment of changes such as resource allocation, job environment, efficiency mismatch between the author and the reviewer, and even their relations. Some of these may be addressed well by the early intervention of the management and thus revert the result of a particular review-iteration. Thus the company may save lots of time and resources.


\subsection{Implication for the practitioners}
The code review process requires serious effort and also is time-consuming. The authors and reviewers involved in a review iteration are likely to get frustrated if they see that their effort goes in vain, i.e., a patchset has to be abandoned, wasting their efforts for quite some time. If they get an early indication from our tool that their current review process is going in a negative direction, they may become cautious, seek external/management help, or at least be prepared mentally. If the management makes a decision early, their efforts would be saved. Thus it would benefit the practitioners.  

\subsection{Implication for Software Engineering Research}
Prior SE researchers followed different approaches including statistical
methods, parametric models, and machine learning (ML) methods for software
effort and duration prediction \cite{shepperd2001using}, software cost
prediction \cite{jorgensen2007systematic}, software fault or defect prediction
\cite{hall2012systematic,shepperd2014researcher}, etc. Search-based peer
reviewer recommendation \cite{ouni2016search} is another related area. Different
prediction models were introduced in the SE (Software Engineering) domain such as predicting the question
quality \cite{baltadzhieva2015predicting} and response time
\cite{goderie2015eta} in Stack Overflow. In these models, the authors exploit
the interactions among users in different contexts related to software
engineering. Bosu et al. \cite{bosu2015characteristics} identified factors that lead to
useful code reviews. Some prior research suggests that a higher number of
reviewers reduces the number of bugs and increases the probability of
acceptability \cite{bavota2015four,kononenko2015investigating}. The experience of
the reviewers sometimes leads to useful code changes
\cite{kononenko2015investigating,baysal2013influence}.

Code review is a very important aspect of modern software engineering. Large
software companies as well as Open Source projects are practicing it with care.
Researchers are trying to generate insight from large repositories of code
review and try to bring efficiency in the process to save the cost of production. In
this work, we study a relatively under-studied problem of predicting whether a
code change will eventually be merged or abandoned at an early stage of the code
review process. We design a machine learning model to apply carefully selected
features generated as a result of communication between the developers and the
reviewers. Our developed tool PredCR is expected to save wastage of effort or
help to recover from being abandoned by inviting early intervention of the
management.

%\anindya{I think you should discuss 2/3 of most similar works and what their limitations are. For example, some of those could be predicted at the end when it is not of much use. The others missed some important features. From this background, you may formulate your specific objective. Also, as background, you may show the parameters of the code review process in a diagram that will give insight that an ML model can predict using features derived from those. Also, you may add some examples that PredCR could successfully predict along with their important feature values.}



%%Code review is a costly and time-consuming task. Besides, it is not feasible to review all the changes with limited resources. Hence, Prioritizing code review is beneficial for proper resource utilization. Our tool can prioritize the review requests based on the score provided by the tool. From that score, the management can easily find out which changes have a higher probability of merging into the main codebase. We propose considering the tool's outcome as a first performance metric for a project. Hence, if the management takes decisive action early based on the prediction, it can significantly improve the decision's quality.   



==> motivation.tex <==
\section{Background and Motivation}
\label{sec:background_motivation}
% \gias{IMPORTANT: for each example, draw a figure or give a visualized example
% to highlight. Right now it's difficult to understand/appreciate the novelty of
% this paper compared to previous works}


Prior SE researchers followed different approaches including statistical
methods, parametric models, and machine learning (ML) methods for software
effort and duration prediction \cite{shepperd2001using}, software cost
prediction \cite{jorgensen2007systematic}, software fault or defect prediction
\cite{hall2012systematic,shepperd2014researcher}, etc. Search-based peer
reviewer recommendation \cite{ouni2016search} is another related area. Different
prediction models were introduced in the software engineering domain such as 
predicting the question quality \cite{baltadzhieva2015predicting} and response time
\cite{goderie2015eta} in Stack Overflow. In these models, the authors exploit
the interactions among users in different contexts related to software
engineering.

Code review is a very important aspect of modern software engineering. Large
software companies as well as Open Source projects are practicing it with care.
Researchers are trying to generate insight from large repositories of code
review and try to bring efficiency in the process to save the cost of production. In
this work, we study a relatively under-studied problem of predicting whether a
code change will eventually be merged or abandoned at an early stage of the code
review process. We design a machine learning model that applies carefully selected
features generated as a result of communication between the developers and the
reviewers. Our developed tool PredCR is expected to save wastage of effort or
help to recover from being abandoned by inviting early intervention of the
management.

\anindya{I think you should discuss 2/3 of most similar works and what their limitations are. For example, some of those could be predicted at the end when it is not of much use. The others missed some important features. From this background, you may formulate your specific objective. Also, as background, you may show the parameters of the code review process in the diagram that will give insight that an ML model can predict using features derived from those. Also, you may add some examples that PredCR could successfully predict along with their important feature values.}

Bosu et al. \cite{bosu2015characteristics} identified factors that lead to
useful code reviews. Some prior research suggests that a higher number of
reviewers reduces the number of bugs and increases the probability of
acceptability \cite{bavota2015four,kononenko2015investigating}. The experience of
the reviewers sometimes leads to useful code changes
\cite{kononenko2015investigating,baysal2013influence}.


% \textcolor{red}{- provide one example to show how and why reviewer dimension
% is important and how it can improve performance over Fan et al. paper.}

In project OpenStack change id 745519
\footnote{https://review.opendev.org/\#/c/745519/}, the reviewer suggested that
the change made by the author is unnecessary (Figure
\ref{fig:abandoned_for_review}). Because a better alternative already exists.
The experienced reviewer knew about this method, but the author did not. After
the reviewer's suggestion, he abandoned the change.

\begin{figure}
\centering
  \includegraphics[width=\linewidth]{images/abandoned_after_review.png}
  \caption{Abandoned after review}
\label{fig:abandoned_for_review}
	\vspace{-6pt}
\end{figure}


In project OpenStack change id 745519 \footnote{https://gerrit.libreoffice.org/c/core/+/65890}, the author was facing build failures because one of the pipeline tests was failing (Figure \ref{fig:abandoned_for_build_fail}). The reviewer mentioned that the test fail is not because of the author's change. If he uploads a new revision of this patch, hopefully, the tests will run successfully. 

\begin{figure}
\centering
  \includegraphics[width=\linewidth]{images/abandoned_after_build_fail.png}
  \caption{Abandoned after build fail}
\label{fig:abandoned_for_build_fail}
	\vspace{-6pt}
\end{figure}

The author later abandoned this change and created another change 66203 \footnote{https://gerrit.libreoffice.org/c/core/+/66203} for the same issue. This was later merged successfully with further helps from the reviewer. Reviewer's experience directly influenced the outcome of these changes.


% \textcolor{red}{- provide one example for this claim ``Also Gerrit
% change requests can have multiple revisions, but Fan et al.
%  predict code change request outcome only at the initial
% submission. Which would not reward change requests which
% was bad during initial submission but improved at a later
% revision.''} 

Many of the changes are not ready for review during the initial submission. The reasons can be 1. build failure 2. pipeline test failure 3. work in progress 4. merge conflict 5. unintentionally included changes 6. dependent on any other change. For this, the author has to push more patch sets. Multiple patch sets are already uploaded before the review even starts. A merge prediction made only on the first patch set would miss any of these cases. For example, in project Eclipse change id 167412 \footnote{https://git.eclipse.org/r/c/platform/eclipse.platform.swt/+/167412}, the initial patch set was set to work in progress (Figure \ref{fig:merged_after_revisions}). The second patch set faced a build fail. On the third patch set, it was set to ready-for-review and finally merged after the eighth patch set. In project LibreOffice change id 100373 \footnote{https://gerrit.libreoffice.org/c/core/+/100373}, it took the author five patch sets to fix build fail. Only then the change was review ready and finally merged at the sixth patchset.

\begin{figure}
\centering
  \includegraphics[width=\linewidth]{images/merged_after_several_revisions.png}
  \caption{Merged after several revisions}
\label{fig:merged_after_revisions}
	\vspace{-6pt}
\end{figure}

% https://gerrit.libreoffice.org/c/core/+/100408 

Fan et al. \cite{fan2018early} found that the author's experience and collaboration activities are the most important factors in predicting the merged probability of a code change in their model. However, this introduced a significant bias against new contributors (less than ten previous changes) in their work. The model was inclined to predict a new contributor's code change as abandoned. To deal with this the authors had to provide an adjusted approach by training and testing separate models from experienced and new contributors. Though collaborative factors influence review outcome \cite{zanetti2013categorizing} \cite{baysal2013influence}, in our model we have compromised by not using the collaboration dimension. So there was less bias towards experienced reviewers. We have added the reviewer dimension, which showed to greatly influence review outcome. Hence the model performance did not fall, rather improved. 

